How Molecules Impact Cells: Unlocking Contrastive PhenoMolecular Retrieval

Predicting molecular impact on cellular function is a core challenge in therapeutic design. Phenomic experiments, designed to capture cellular morphology, utilize microscopy based techniques and demonstrate a high throughput solution for uncovering molecular impact on the cell. In this work, we learn a joint latent space between molecular structures and microscopy phenomic experiments, aligning paired samples with contrastive learning. Specifically, we study the problem ofContrastive PhenoMolecular Retrieval, which consists of zero-shot molecular structure identification conditioned on phenomic experiments. We assess challenges in multi-modal learning of phenomics and molecular modalities such as experimental batch effect, inactive molecule perturbations, and encoding perturbation concentration. We demonstrate improved multi-modal learner retrieval through (1) a uni-modal pre-trained phenomics model, (2) a novel inter sample similarity aware loss, and (3) models conditioned on a representation of molecular concentration. Following this recipe, we propose MolPhenix, a molecular phenomics model. MolPhenix leverages a pre-trained phenomics model to demonstrate significant performance gains across perturbation concentrations, molecular scaffolds, and activity thresholds. In particular, we demonstrate an 8.1x improvement in zero shot molecular retrieval of active molecules over the previous state-of-the-art, reaching 77.33% in top-1% accuracy. These results open the door for machine learning to be applied in virtual phenomics screening, which can significantly benefit drug discovery applications.

==> archive_experiments.tex <==


% \begin{figure}[b]
%     \centering
%     \includegraphics[width=.95\textwidth]{figs/MolPhenix_v3.pdf}
%     \caption{Illustration of proposed guidelines when incorporated in our \textit{MolPhenix} contrastive phenomic retrieval framework. We address challenges by utilizing a uni-modal pretrained MAE \& MPNN models, inter-sample weighting with a dosage aware \texttt{S2L} loss, undersampling inactive molecules, and encoding molecular concentration.}
%     \label{fig:main}
% \end{figure}


\section{Methodology}

In this section, we explain key challenges facing phenomolecular retrieval and provide guidelines that are key methodological improvements behind the success of MolPhenix \ref{fig:main}.


\textbf{Preliminaries:} Our setting studies the problem of learning multi-modal representations of molecules and phenomic experiments of treated cells \cite{cloome}. The aim of this work is to learn a joint latent space which maps phenomic experiments of treated cells and the corresponding molecular perturbations into the same latent space. We consider a set of lab experiments $\mathcal{E}$ defined as the tuple ($\mathbf{X}, \mathbf{M}, \mathbf{C}, \mathbf{\Psi}$). Each experiment $\epsilon \in \mathcal{E}$ consists of data samples $\mathbf{x}_{i} \in \mathbf{X}$ (such as images) and perturbations $\mathbf{m}_{i} \in \mathbf{M}$ (such as molecules) which are obtained at a specific dosage concentration $\mathbf{c}_{i} \in \mathbf{C}$.

Figure \ref{fig:contrastive_phenomolecular_retrieval} describes the problem of contrastive phenomolecular retrieval, where for a single image \(\mathbf{x}_i\), the challenge consists of identifying the matching perturbation,  \(\mathbf{m}_i\), and concentration, \(\mathbf{c}_i\), used to induce morphological effects on the cell.
This can be accomplished in a zero-shot way by generating embeddings for \((\mathbf{m}_1, \mathbf{c}_1),... (\mathbf{m}_j, \mathbf{c}_j)\) and \(\mathbf{x}_i\) using functions \(f_{{\theta}_m}(\mathbf{m}, \mathbf{c})\) \(f_{{\theta}_x}(\mathbf{x})\) which map samples into \(\mathbb{R}^d\).
\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-.2cm}
\begin{center}
    \includegraphics[width=0.5\textwidth]{figs/phenomolecular_retrieval.pdf}
    \caption{Illustration of the contrastive phenomolecular retrieval challenge. Image \(\mathbf{x}_i\) and a set of molecules and corresponding concentrations \((\mathbf{m}_k, \mathbf{c}_k)\) get mapped into a \(\mathbb{R}^d\) latent space. Their similarities get computed with \(f_{\sim}\) and ranked to evaluate whether the paired perturbation appears in the top K\%.}
    \label{fig:contrastive_phenomolecular_retrieval}
\end{center}
\vspace{-0.75cm}
\end{wrapfigure}
Then, by defining a similarity metric between generated embeddings \(\mathbf{z}_{x_i}\) and \(\mathbf{z}_{m_i}\), \(f_{sim}\), we can rank \((\mathbf{m}_1, \mathbf{c}_1)... (\mathbf{m}_j, \mathbf{c}_j)\) based on computed similarities. An effective solution to the contrastive phenomolecular retrieval problem would learn \(f_{{\theta}_m}(\mathbf{m}, \mathbf{c})\) and \(f_{{\theta}_x}(\mathbf{x})\) that results in consistently high retrieval rates of \((\mathbf{m}_i, \mathbf{c}_i)\) used to perturb \(\mathbf{x}_i\).

In practice, the image embeddings are generated using a phenomics microscopy foundation MAE model. We use phenomic embeddings to marginalize batch effects, infer inter-sample similarities, and undersample inactive molecules. For each sample, a $p$ value cutoff $\psi \in \mathbf{\Psi}$ denotes the threshold of molecular activity. Molecules below the $p$ value cutoff $\psi$ are considered active, while molecules above $\psi$ are considered as inactive. 
% We explore a multitude of different methods to encode of molecular concentration (such as \texttt{one-hot} or \texttt{sigmoid}). 

Prior methods in multi-modal contrastive learning utilize the InfoNCE loss, and variants thereof \cite{infonce} to maximize the joint likelihood of \(\mathbf{x}_i\) and \(\mathbf{m}_i\). Given a set of $N \times N$ random samples \((\mathbf{x}_{1}, \mathbf{m}_{1}, \mathbf{c}_{1}), \cdots, (\mathbf{x}_{N}, \mathbf{m}_{N}, \mathbf{c}_{N})\) containing $N$ positive samples at $k^{\text{th}}$ index and $(N-1) \times N$ negative samples, optimizing Equation \ref{eq:infonce} maximizes the likelihood of positive pairs while minimizing the likelihood of negative pairs:

%  Figure out what the expectation is over
\begin{equation}
    \mathcal{L}_{\text{InfoNCE}} = - \frac{1}{N}\sum_{i=1}^N
    \left[ \log \frac{
    \exp(\langle \mathbf{z}_{x_i}, \mathbf{z}_{m_i} / \tau \rangle)
    }{
    \sum_{k = 1}^{N} \exp(\langle \mathbf{z}_{x_i}, \mathbf{z}_{m_k} / \tau \rangle) + 
    \sum_{k = 1}^{N} \exp(\langle \mathbf{z}_{m_i}, \mathbf{z}_{x_k} / \tau \rangle)
    } \right] 
    \label{eq:infonce}.
\end{equation}

Where \(\mathbf{z}_{x}\), \(\mathbf{z}_{m}\) correspond to phenomics and molecular embeddings respectively, \(\tau\) is softmax temperature,  and \(\langle \cdot \rangle\) corresponds to cosine similarity.

\subsection*{Challenge 1: Phenomic Pretraining and Generalization}

% Topic sentence
We find that using a phenomics foundation model to embed microscopy images allows for mitigation of batch effects, reduces the required number of paired data points, and improves generalization in the process. 
% Similar to text-image multi-modal training, contrastive phenomolecular retrieval involves mapping paired samples from distinct modalities to the same point in the learned latent space. 
 % Expand on data availability challenge
 While \texttt{CLIP}, a hallmark model in the field of text-image multi-modality, was trained on 400 million curated paired data points, there is an order of magnitude fewer paired molecular-phenomic molecule samples \cite{clip}. 
Cost and systematic pre-processing of data make large scale data generation efforts challenging, and resulting data is affected by experiment specific batch effects.
\textbf{Batch effects} induce noise in the latent space as a result of random perturbations in the experimental process, while biologically meaningful variation remains unchanged, making it difficult to find correlations within the data distribution \cite{batcheffect2,batcheffect3}. 
Limited dataset sizes and batch effects make it challenging for contrastive learners to capture the relationships that drive molecular effects on cells, yielding to low retrieval accuracies \cite{cloome}.

 % Wrap up with generalization challenges
%The above difficulties are further amplified in downstream generalization when evaluating model zero-shot generalization. Multi-modal molecular-phenomic models struggle to demonstrate positive transfer on unseen molecules, phenomic experiments and dosage concentrations. This occurs due to the inability of contrastive learners to capture inter-atomic relationships that drive the molecular effect on cells. 
% Instead, such models overfit to image modality priors and struggle to recuperate from locally suboptimal representations.

 %Our solution for taking a pre-trained model and multi stage generalization evaluation
We address data availability and generalization challenges by utilizing representations from a large \textbf{uni-modal pre-trained phenomic model}, $\theta_{\text{Ph}}$, trained to capture an expressive representation of cellular data. $\theta_{\text{Ph}}$ is pretrained on raw microscopic images using a Fourier modified MAE objective, utilizing the ViT-L/8 architecture \cite{mae,vit}. For simplicity, we refer to this model as \textit{Phenom-1} in future sections \cite{ph1,kraus2024masked}. This pretrained model allows a drastic reduction in the required number of paired multi-modal samples \cite{zhai2022lit}. In addition, using phenomic representations alleviates the challenge of batch effects by averaging samples, \(\mathbf{z}_{x}\), generated with the same perturbation \(\mathbf{m}_i\) over multiple lab experiments \(\epsilon_i\). Averaging model representations \(\frac{1}{N} \Sigma^1_{i \in N} \mathbf{z}_{x_i}\) allows marginalizing batch effect induced by individual experiments.

%Guideline \ref{th:one} summarizes utilizing pretrained uni-modal models as a remedy.

\begin{tcolorbox}
\begin{theorem}
\label{th:one}
When training a molecular-phenomic model, utilizing pre-trained uni-modal encoder, $\theta_{\text{Ph}}$, can be used to reduce the number of paired data-points to achieve matched retrieval performance, and averaging phenomic embeddings \(\mathbf{z}_{\text{Ph}}\) from matched perturbation samples can alleviate batch effects.
\end{theorem}
\end{tcolorbox}

While Phenom-1 serves as an effective prior for phenomic experiments, certain models can be used to reason over molecular structures by leveraging additional inductive biases. Thus, we make use of features learned from GNNs trained on molecular property prediction \cite{gps++}. Specifically, we utilize a pretrained MPNN foundational model up to the order of 1B parameters for extracting molecular representations. We refer to this model as \textit{MolGPS} \cite{molgps}.

\subsection*{Challenge 2: Inactive Molecular Perturbations}

\begin{wrapfigure}{r}{0.4\textwidth}
\vspace{-1.75cm}
\begin{center}
    \includegraphics[width=0.37\textwidth]{figs/no_perturbation_figure.png}
    \caption{Data generation process of a phenomic experiment on cells \( \mathbf{x_i} \) with molecular perturbations \( \mathbf{m_i} \) and concentrations \( \mathbf{c_i} \).}
    \label{fig:no_molecular_effect}
\end{center}
\vspace{-0.75cm}
\end{wrapfigure}

% Describe the challenge intuitively and then provide a mathematical formulation
% We now focus on the challenge of perturbations arising from inactive molecules in cases where the molecule has no effect on the morphology of the perturbed cells. 
The phenomics-molecular data collection process can result in pairing of molecular structures with unperturbed cells in cases where the molecule has no effect on cell morphology \ref{fig:no_molecular_effect}. 
Since the molecular effects observed in cell \(\mathbf{x}_i\) is conditioned on the perturbation, then in cases of an absence of molecular effect \(P(\mathbf{x_i} | \mathbf{x}^0_i, \mathbf{c_i}, \mathbf{m_i}) \sim P(\mathbf{x_i} | \mathbf{x}^0_i)\). In these cases, the cellular samples will be independent, from paired molecular data, which results in paired data being misannotated under the assumption of data-pairs having an underlying biological relationship. This can make training of contrastive phenomic-molecular models challenging. We demonstrate how utilizing Phenom-1 to undersample inactive molecules and learn continuous similarities between samples can alleviate this challenge.

% We use p-value thresholding 
To \textbf{undersample inactive molecules}, we extract the embeddings from Phenom-1 and calculate the relative activity of each perturbation \(\mathbf{m_i} \in \mathbf{M}\). This is done using the rank of cosine similarities between technical replicates produced for a molecular perturbation against a null distribution. The null distribution is establishing by calculating cosine similarities from random pairs of Phenom-1 embeddings generated with perturbation \(m_j, m_k\). Hence, we can compute a p-value \(\psi\) and filter out samples likely to belong to the null distribution with an arbitrary threshold $\psi$.

% Use a specialized loss
In this second strategy, we present the custom \textbf{S2L training objective}, which alleviates the challenge of inactive molecular perturbations. 
S2L is grounded in previous work which demonstrates improved robustness to label noise and makes use of inter-sample similarities \cite{siglip, cwcl}. 
Continuous Weighted Contrastive Learning (CWCL) provides better multi-modal alignment using a uni-modal pretrained model to suggest inter-sample distances, relaxing the negative equidistant assumption present in InfoNCE \cite{cwcl}: 

\begin{equation}
    \mathcal{L}_{\text{CWCL}, \: \mathcal{U} \rightarrow \mathcal{V}} = - \frac{1}{N}\sum_{i=1}^N
    \left[ \frac{1}{\sum_{i=j}^{N} \mathbf{w}_{i,j}} \sum_{i=1}^{N} \mathbf{w}_{i,j} \log 
    \frac{ 
    \exp{\left(  \langle \mathbf{z}_{x_i},\mathbf{z}_{m_j} \rangle / \tau \right) }}
    { \sum_{k=1}^{N} \exp{ \left( \langle \mathbf{z}_{x_j}, \mathbf{z}_{m_k} \rangle / \tau \right) }} \right]. \label{eq:cwcl}
\end{equation}

CWCL logit weighting with a continuous measure of similarity $\mathbf{w}$, results in better alignment of embeddings $\mathbf{z}_{\mathbf{x}_{i}}$ and $\mathbf{z}_{\mathbf{m}_{j}}$ across modalities. In equation \ref{eq:cwcl}, \(\mathbf{w}\) is computed using an within modality similarity function such as \( w_{i,j} = \langle z_{\mathbf{x}_i}, z_{\mathbf{x}_j} \rangle / 2 + 0.5 \). Note, the above formula is used only for modality \(\mathcal{U}\) for which a pre-trained model is available.

Another work, SigLIP, demonstrates robustness to label noise and reduces computational requirements during contrastive training \cite{siglip}. It does so by avoiding computation of a softmax over the entire set of in-batch samples, instead relying on element-wise sigmoid operation:

\begin{equation}
    \mathcal{L}_{\text{SigLIP}} = 
    - \frac{1}{N}
    \sum_{i=1}^N 
    \sum_{i=j}^N
    \left[ \log 
    \frac{1}{1 + \exp{ \left( \mathbf{y}_{i,j}(-\alpha \: \langle \mathbf{z}_{\mathbf{x}_{i}}, \mathbf{z}_{\mathbf{m}_{j}} \rangle + b) \right) }}
    \right]. \label{eq:siglip}
\end{equation}

In equation \ref{eq:siglip}, \(\alpha\) and \(b\) are learned, hence calibrating the model confidence conditioned on the ratio of positive to negative pairs.

Since the two objectives complement each other and their combined effects mitigate weak or inactive perturbations appearing in our dataset, we combine them for molecular representation learning. This yields the S2L training objective:

\begin{equation}
    \mathcal{L}_{\text{S2L}} =  
    - \frac{1}{N}
    \sum_{i=1}^N 
    \sum_{i=j}^N
    \log \left[ 
    \frac{\mathbf{w}_{i,j}}
    {1 + \exp{ \left( -\alpha \mathbf{z}_{\mathbf{x}_{i}}.\mathbf{z}_{\mathbf{m}_{j}} + b) \right) }} +
    \frac{(1 - \mathbf{w}_{i,j})}
    {1 + \exp{ \left( \alpha \mathbf{z}_{\mathbf{x}_{i}}.\mathbf{z}_{\mathbf{m}_{j}} + b) \right) }} 
    \right]. \label{eq:s2l}
\end{equation}

In the equation above, \(\mathbf{z}_{\mathbf{x}_i}\) and \(\mathbf{z}_{\mathbf{m}_j}\) correspond to latent representations of images and molecules, respectively. \(\alpha\) and \(\
b\) correspond to learnable temperature and bias parameters for the calibrated sigmoid function. \(\mathbf{w}_{ij}\) is an inter-sample similarity function computed from images using the pretrained model \(\theta_{\text{Ph}}\). To compute \(\mathbf{w}_{i,j}\), we use the arctangent of L2 distance instead of a modified cosine similarity as was the case for Equation \ref{eq:cwcl} (more details in Appendix \ref{sec:s2l_distance_appendix}). Intuitively, S2L can be thought of as shifting from a multi-class classification to a soft multi-label problem. Here, the labels are continuous and determined by sample similarity in the phenomics space.


\begin{tcolorbox}
\begin{theorem}
\label{th:two}
When training a molecular-phenomic model, mitigating the effect of inactive molecules in training data distribution can be carried out by undersampling inactive molecules and using an inter-sample similarity aware, \texttt{S2L} loss.
\end{theorem}
\end{tcolorbox}

\subsection*{Challenge 3: Variable Concentrations}

% Topic sentence indicating that molecular impact is a function of molecule dosage 
% As well as perturbation identity
Perturbation effect on a cell is determined by both molecular structure and corresponding concentration \cite{carcinogenicity_dosage}. A model capturing molecular impact on cell morphology must be able to generalize across different concentrations, since variable concentrations for the same molecule correspond to different data distributions.

We note that providing concentrations $\mathbf{c}_{i}$ as input to the model would benefit performance, as this would make the model aware of cell activity. However, we find that simply concatenating or learning concentrations does not result in effective training. To that end, we add concentration information in two separate ways: \textit{implicit} and \textit{explicit} formulations.

We add \textbf{implicit concentration}  as molecular perturbation classes by using the S2L loss (introduced in the previous section) to treat perturbation \(\mathbf{m}_i\) with concentrations \(\mathbf{c}_i\) and \(\mathbf{c}_j\) as distinct classes. This pushes samples apart in the latent space proportionally to their phenomic similarities.

We add \textbf{explicit concentration}  $c_{i}$ by passing it to the molecular encoder. In order to prevent overfitting towards multi-modal inputs, we provide encoded representations of dosage concentrations $\mathbf{f'}(c_{i})$ as inputs $\mathbf{f'}: \mathcal{C} \rightarrow \mathbb{R}$ as a functional mapping. 
Encoded representations $\mathbf{f}(c_{i})$ are concatenated at the initial layer of the model.
While one may choose to learn the mapping $\mathbf{f}$, we found simpler functional encodings (such as \texttt{one-hot} and \texttt{logarithm}) to work well in practice. % Guideline \ref{th:three} presents our remedy for tackling variable concentration training.


\begin{tcolorbox}
\begin{theorem}
\label{th:three}
When training a molecular-phenomic model, conditioning on an (implicit or explicit) representation of concentration $\mathbf{f'}(c_{i})$ aids in capturing molecular impacts on cell morphology and improves model generalization to previously unseen molecules and concentrations.
\end{theorem}
\end{tcolorbox}



==> archive_introduction.tex <==
\section{Introduction}


Quantifying cellular responses elicited by genetic and chemical perturbations represents a core challenge in medicinal research \cite{cell_impact1, cell_impact2}. Microscopy-based screening techniques allow a comprehensive understanding of a molecule's biological effects \cite{image-profiling, cell_painting}. Molecules with similar properties share such biological effects. Hence, retrieving representations of unseen but similar molecules aids in the discovery of novel therapeutic drug candidates \cite{extracted_feature_method, HCS-deep-learning, HCS-deep-learning2}.

\textit{Contrastive Phenomic Retrieval} is one such avenue of constructing and storing learned representations of molecules \cite{cloob, surv_contrastive, better_features_contrastive}. Molecular information is retrieved from a joint embedding space of phenome images and molecule fingerprints constructed using multi-modal contrastive learning. Unlike text-image retrieval, molecular retrieval struggles from three main challenges. Firstly, molecular modalities such as images and atomic fingerprints have a more intricate relationship on properties of the molecule. This requires a more compact and well-structured latent space. Secondly, a scarcity of large molecular datasets makes it challenging to obtain screened cell pairs and their chemical structures. This inhibits generalization and transfer to unseen cellular images, compound structures and dosage concentrations. Lastly, latent variables must capture the effect of compounds on various cell states. Inactive molecules that do not effect cell states are categorized as negative samples since they do not demonstrate a positive pairing. This leads to a large number of negative samples destabilizing the learning procedure.

Prior efforts in contrastive phenomic retrieval have utilized learned knowledge bases and compact representations of molecules. Modalities such as images and molecular fingerprints are first stored in the latent space of customized encoders and retrieved using downstream contrastive learning \cite{phenome1, cloome}. Although effective, these methods require the use of hand-engineered contrastive losses which succumb to label noise and fail to generalize in OOD settings. Retrieved molecules undergo the phenomenon of \textit{batch effect} wherein random perturbations in cell compositions affect predictions of the model \cite{bacheffect1, batcheffect2, batcheffect3}. The presence of batch effect and generalization bottlenecks make it unclear on which design decisions are pivotal. Furthermore, a lack of understanding of these design decisions make them challenging to incorporate in a real-world experimental laboratory with computational constraints and limited cell lifetimes.

We explore retrieval of phenomic molecules by understanding the behavior of contrastive learning methods in the presence of unseen data samples. Our study focusses on identifying the key factors which influence contrastive learning over seen and unseen molecules. Towards this goal, we uncover five key \textit{ingredients} required to accelerate and improve retrieval of new molecules across different modalities such as images, embeddings and molecular fingerprints. Specifically, contrastive learners demonstrate higher retrieval rates when (1) bootstrapped with a pretrained model, (2) weighted contrastive learning is combined with a sigmoid loss, (3) active molecules are oversampled, (4) models are conditioned on an encoded representation of dosage and (5) a universal evaluation criterion is adopted. 

Following these guidelines, we build MolPhenix and  demonstrate consistent improvements in the presence of batch effect across different dosage concentrations, molecule types and cutoff thresholds. 
Additionally, MolPhenix outperforms base methods in zero-shot and few-shot transfer on unseen molecules, even in the presence of small parameter size constraints. \db{Indeed, MolPhenix achieves 75\% top-1\% retrieval of unseen molecules, a 9X improvement over reported results in \cite{cloome}. ADD OTHER IMPRESSIVE RESULTS HERE.}


==> archive_methodology.tex <==


\section{Navigating Challenges in Contrastive Phenomic Retrieval}


\begin{wrapfigure}{r}{0.35\textwidth}
\vspace{-0.5cm}
\begin{center}
    \includegraphics[width=0.34\textwidth]{figs/phenome_experiment.png}
    \caption{Lab experiment obtaining phenome molecules. Single-cell phenome images and embeddings are extracted from whole genome using microscopy imaging.}
    \label{fig:experiment}
\end{center}
\vspace{-0.5cm}
\end{wrapfigure}

\textbf{Preliminaries:} Our setting studies the problem of learning multi-modal representations of phenome cells \cite{cloome}. We consider a set of lab experiments $\mathcal{E}$ defined as the tuple ($\mathbf{X}, \mathbf{S}, \mathbf{C}, \mathbf{\Psi}$). Each experiment $\epsilon \in \mathcal{E}$ consists of unlabelled data samples $\mathbf{x}_{i} \in \mathbf{X}$ (such as images) and $\mathbf{s}_{i} \in \mathbf{S}$ (such as sensor readings or embeddings) which are obtained at a specific dosage concentration $c_{i} \in \mathbf{C}$. Figure \ref{fig:experiment} presents the illustration of an experiment wherein phenome images extracted using microscopy imaging correspond to $\mathbf{x}_{i}$. Their embeddings extracted from a VAE prior correspond to $\mathbf{s}_{i}$. Each experiment corresponds to a $p$ value cutoff $\psi \in \mathbf{\Psi}$ which denotes the threshold of molecular activity. Molecules below the $p$ value cutoff $\psi$ are considered active while molecules above $\psi$ are considered as inactive. A molecular model, and its parameters $\theta$, aim to learn a mapping $\mathcal{Z}: \mathbf{X} \times \mathbf{S} \rightarrow \mathbb{R}$ where $\mathbf{z}_{i} = \theta(\mathbf{x}_{i}, \mathbf{s}_{i}, \mathbf{f}(c_{i}))$, $\mathbf{f}(c_{i})$ is an encoding of the dosage concentration (such as \texttt{one-hot} or \texttt{sigmoid}) and $\mathbf{y}_{i}$ is the label. We denote embeddings of modality $\mathbf{x}_{k}$ with $\mathbf{z}_{\mathbf{x}_{k}}$ and embeddings of modality $\mathbf{s}_{k}$ with $\mathbf{z}_{\mathbf{s}_{k}}$. We explicitly represent models of phenomic cells as $\theta_{Ph}$ with their number of parameters as $|\theta_{Ph}|$. Prior methods in contrastive learning utilize the InfoNCE loss \cite{infonce} to maximize likelihood of positive logits. Given a set of $N$ random samples [$\theta(\mathbf{x}_{1}, \mathbf{s}_{1}, \mathbf{f}(c_{1})), \theta(\mathbf{x}_{2}, \mathbf{s}_{2}, \mathbf{f}(c_{2})), \cdots, \theta(\mathbf{x}_{N}, \mathbf{s}_{N}, \mathbf{f}(c_{N}))$] containing one positive sample at $k^{\text{th}}$ index and $N-1$ negative samples, we optimize the functional in Equation \ref{eq:infonce}.

\begin{equation}
    \mathcal{L}_{\text{InfoNCE}} = - \mathbb{E}_{\mathbf{x}_{k} \sim \mathbf{X}, \mathbf{s}_{k} \sim \mathbf{S}, \mathbf{c}_{k} \sim \mathbf{C}} \left[ \log \frac{\theta(\mathbf{x}_{k}, \mathbf{s}_{k}, \mathbf{f}(c_{k}))}{\sum_{i = 1}^{N} \theta(\mathbf{x}_{i}, \mathbf{s}_{i}, \mathbf{f}(c_{i}))} \right] \label{eq:infonce}
\end{equation}


\textbf{$\blacktriangleright$ Challenge 1: Phenomic Pretraining and Generalization}

 Pretraining custom phenome models from scratch poses computational and generalization constraints. On the computational front, model $\theta_{\text{Ph}}$ is tasked to capture features across molecular cell activity and their effect on one another. This requires a greater degree of control and domain-enigneered solutions. On the generalization front, custom phenome models struggle to demonstrate positive transfer towards unseen molecules and dosage concentrations. This occurs due to the inability of contrastive learners to capture inter-atomic relationships between inactive molecules. Such models overfit to image modality priors and struggle to recuperate from locally suboptimal representations.

We address prior challenges in generalization by taking a data-driven approach. The key intuition behind our approach is that bootstrapping from a larger phenomic model must bake in a general structure about the relationship of cells and their effects on one another. We acquire pretrained representations from a high-capacity generalist phenomic model $\theta$ and utilize them for training custom phenomic contrastive learners. Such a high-capacity model is pretrained on raw microscopic images of single-cell phenome molecules extracted from the whole genome map. While we do not impose constraints on training schemes of these models, we note that bootstrapping from $\beta$-VAE models is computationally efficient as these trade-off the number of parameters for representation disentanglement. Guideline \ref{th:one} summarizes bootstrapping as a remedy.

\begin{theorem}
\label{th:one}
When training a phenome model $\theta_{\text{Ph}}$, bootstrapping embeddings $\mathbf{z_{i}}$ from a high-capacity pretrained model $|\theta| > |\theta_{Ph}|$ aids in  accelerating training.
\end{theorem}

While $\beta$-VAEs serve as a simple prior, certain models can reason about the structure of molecules by leveraging additional inductive biases. Thus, we take the above idea a step further and bootstrap aggregated feature readouts from GNNs \cite{gps++}. Specifically, we utilize pretrained foundational models upto the order of 1B parameters for extracting molecular representations \cite{molgps}. We follow the analysis of \cite{molgps} and scale both depth and width in MPNN architectures. While a larger parameter count induces a general structure, message-passing provides us with expressive molecular representations.

\textbf{$\blacktriangleright$ Challenge 2: Randomized Batch Effects}

Bootstrapping from a pretrained model aids in generalization, however downstream models still struggle from the curse of \textit{batch effect}. Batch effects induce random noise in the latent space as a result of random perturbations experienced by cell compositions \cite{batcheffect2}. Cell clusters exhibit shifts in their position and orientation while their underlying molecular properties remain unchanged. This creates distortion across modalities and embeddings wherein the same molecular conformation in latent space may be mapped to different cell attributes \cite{batcheffect3}.

A naive solution to this problem dictates averaging recorded samples over multiple lab experiments. In the case of contrastive learning, this would correspond to averaging learned representations from our bootstrapped model $\theta$. In practice, this has little effect in the presence of large datasets containing samples from multiple modalities. We thus focus on directly improving the loss function.

Prior work has focussed on stabilizing training using Continuous Weighted Contrastive Learning (CWCL) \cite{cwcl}. Weighing logits with a continuous measure of similarity $\mathbf{w}$ results in better alignment of embeddings $\mathbf{z}_{\mathbf{x}_{k}}$ and $\mathbf{z}_{\mathbf{s}_{k}}$ across modalities. On the other hand, the more recent work of Sigmoid loss for Language-Image Pretraining (SigLIP) \cite{siglip} mitigates the requirement of global views of samples $\mathbf{z}_{\mathbf{x}_{k}}$ and $\mathbf{z}_{\mathbf{s}_{k}}$.

\begin{equation}
    \mathcal{L}_{\text{CWCL}} = - \mathbb{E}_{\mathbf{z}_{\mathbf{x}}, \mathbf{z}_{\mathbf{x}}} \left[ \frac{1}{\sum_{i=1}^{N} \mathbf{w}_{i}} \sum_{i=1}^{N} \mathbf{w}_{i} \log \frac{ \exp{ \left( \mathbf{z}_{\mathbf{x}_{i}}.\mathbf{z}_{\mathbf{x}_{i}} / \tau \right) }}{ \sum_{j=1}^{N} \exp{ \left( \mathbf{z}_{\mathbf{x}_{j}}.\mathbf{z}_{\mathbf{x}_{j}} / \tau \right) }} \right]
\end{equation}
\begin{equation}
    \mathcal{L}_{\text{SigLIP}} = - \mathbb{E}_{\mathbf{z}_{\mathbf{x}_{k}}, \mathbf{z}_{\mathbf{x}_{k}}} \left[ \log \frac{1}{1 + \exp{ \left( \mathbf{y}_{k}(-\alpha \mathbf{z}_{\mathbf{x}_{k}}.\mathbf{z}_{\mathbf{s}_{k}} + b) \right) }} \right]
\end{equation}

While CWCL provides better multi-modal alignment, SiGLIP mitigates reliance on different molecular conformations. Since the two objectives complement each other and their combined effects mitigate batch effect, we may safely combine them for molecular representation learning. This yields the CWCL+SigLIP loss function presented in Equation \ref{eq:cwclsiglip}.

\begin{equation}
    \mathcal{L}_{\text{CWCL+SigLIP}} =  \label{eq:cwclsiglip}
\end{equation}

The above CWCL+SigLIP combination provides a unified framework for mitigating the batch effect. An intriguing aspect of the loss function is that while positive logits have a higher weighted preference, these preferences scale sub-linearly. Such a smooth transition across logits stabilizes training across multi-modal inputs. Guideline \ref{th:two} provides our remedy for mitigating the batch effect.

\begin{theorem}
\label{th:two}
When training a phenome model $\theta_{\text{Ph}}$, averaging representations across lab experiments $\epsilon \in \mathcal{E}$ and combining contrastive weighted learning with a sigmoid loss using Equation \eqref{eq:cwclsiglip} minimizes susceptibility to randomized batch effects across molecule configurations.
\end{theorem}

\textbf{$\blacktriangleright$ Challenge 3: Inactive Molecule Configurations}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\textwidth]{figs/main.png}
    \caption{Illustration of proposed guidelines when incorporated in a contrastive phenomic retrieval pipeline. We address challenges by bootstrapping from a pretrained MAE/MPNN,  weighting a novel sigmoid loss, oversampling active molecules, encoding dosage concentrations and recommending an unbiased evaluation protocol across cutoff thresholds.}
    \label{fig:main}
\end{figure}
While combining a sigmoid loss with continuous weighting mitigates batch effect, phenomic learners still fall prey to negative samples such as inactive molecules. Since inactive molecules do not share similar chemical or physical structure, these have little to no influence on the embeddings of a bootstrapped model. These molecules inject label noise since molecules may share a range of inter-atomic characteristics with active molecules (e.g- bond lengths and torsional forces). Analogously, the modified loss function of Equation \ref{eq:cwclsiglip} does not take into account the alignment of samples across different classes. We thus need an alternative to tackle the large number of negative samples.

It is a well known phenomenon that increasing the batch size of samples improves performance of contrastive learning models \cite{clip, simclr2}. However, number of positive and negative samples are both increased proportionally to achieve these gains. We take this property a step further and ask \textit{whether increasing the number of positive samples makes contrastive learning robust?} 

Surprisingly, oversampling active molecules as positive samples improves recall from learned embeddings. In addition to inactive molecules above the cutoff threshold $\psi$, we additionally draw samples below the cutoff threshold $\psi$ and add them to our current training batch. This process is repeated for different experiments $\epsilon \in \mathcal{E}$, across different concentrations $\psi \sim \mathbf{\Psi}$ and different modalities $\mathbf{x}_{i}$ and $\mathbf{s}_{i}$. Oversampling active molecules across different concentrations shapes the latent space to be robust to negative outliers (such as inactive molecules structurally similar to active molecules). Guideline \ref{th:three} presents our oversampling strategy.

\begin{theorem}
\label{th:three}
When training a phenome model $\theta_{\text{Ph}}$, oversampling active molecules with cutoff thresholds $\mathbf{\psi} \sim \mathbf{\Psi}$ aids in mitigating noise from inactive molecules.
\end{theorem}

\textbf{$\blacktriangleright$ Challenge 4: Variable Concentrations}

Generalization across different dosage concentrations is a representational bottleneck. Variable dosage concentrations correspond to different data distributions of similar molecules. This prohibits us from treating two instances of the same molecule as a single data sample. Furthermore, dosage concentrations determine the level of cell activity. Higher concentration values indicate cell saturation with limited data samples. Lower concentration values, on the other hand, denote greater number of samples with the majority representing inactive molecules. This creates an unbalanced set of samples where scalar concentration values fail to capture a clear demarcation between cells. Thus, we must inform phenomic models of information contained within different concentrations.

We note that providing dosage concentrations $c_{i}$ as input to the model would benefit performance as this would make the model aware of cell activity. However, simply concatenating or learning concentrations may not result in effective training. Models can simply choose to ignore concentrations $c_{i}$ by treating them as input noise. Thus, in order to prevent overfitting towards multi-modal inputs, we provide encoded representations of dosage concentrations $\mathbf{f}(c_{i})$ as additional inputs to the phenomic model with $\mathbf{f}: \mathcal{C} \rightarrow \mathbb{R}$ being a functional mapping. Encoded representations $\mathbf{f}(c_{i})$ are concatenated at last or penultimate layers of the model. While one may choose to learn the mapping $\mathbf{f}$, we found simpler functional encodings (such as \texttt{one-hot} and \texttt{logarithm}) to work well in practice. Guideline \ref{th:four} presents our recommendation for encoding variable concentrations.

\begin{theorem}
\label{th:four}
When training a phenome model $\theta_{\text{Ph}}$, conditioning on an encoded representation of dosage concentrations $\mathbf{f}(c_{i})$ aids in generalization.
\end{theorem}

\textbf{$\blacktriangleright$ Challenge 5: Universal Evaluation}

So far we have studied improving training of phenomic models. However, evaluating such methods comprehensively is an equally challenging area. With the absence of a universal evaluation scheme, prior works employ different metrics and evaluation protocols \cite{cloom, phenome1}. This inconsistency creates reproducibility and performance bottlenecks wherein evaluating the same model on a new subset of molecules yields inconsistent and widely varying results \cite{rxrx3}.

Additionally, prior works fail to leverage cutoff thresholds which characterize the boundary of molecular activity. Evaluating all molecules corresponding to a single threshold $\psi$ results in a biased estimate of performance. Since cutoff thresholds consist of different number of data samples, evaluation protocols lean towards thresholds with the largest subset of data. We thus require an unbiased estimate of retrieval performance.

Our framework addresses the above challenges by creating a universal evaluation protocol utilizing cutoff thresholds $\psi \in \mathbf{\Psi}$. We recommend evaluating phenomic models on subsets of molecules sampled at different cutoff thresholds $\psi$ in the cutoff threshold set $\mathbf{\Psi}$. Corresponding to each threshold $\psi$, retrieval metrics (such as retrieval accuracy) are tracked and averaged for an unseen set of molecules. This process is repeated for all thresholds in the threshold set $\mathbf{\Psi}$. Finally, metrics are averaged across cutoff thresholds and reported across different random runs. Our evaluation protocol is based on the intuition that a larger cutoff threshold set will yield accurate unbiased estimates of true performance. Mathematically, for a given metric $\mathcal{M}$, our evaluation protocol tracks $\mathfrak{M}$ which is the expected value of $\mathcal{M}$ over all cutoff thresholds.

\begin{equation}
    \label{eq:eval}
    \mathfrak{M}(\theta, \mathbf{X}, \mathbf{S}, \mathbf{\Psi}) = \mathbb{E}_{\psi \sim \mathbf{\Psi}} \left[ \mathbb{E}_{\mathbf{x}, \mathbf{s}} \left[ \mathcal{M}(\theta, \mathbf{x}, \mathbf{s}, \psi) \right] \right] \delequal \mathbb{E}_{\mathbf{x}, \mathbf{s}} \left[ \mathbb{E}_{\psi \sim \mathbf{\Psi}} \left[ \mathcal{M}(\theta, \mathbf{x}, \mathbf{s}, \psi) \right] \right]
\end{equation}


\begin{theorem}
\label{th:five}
When training a phenome model $\theta_{\text{Ph}}$, evaluating the learner on variable cutoff thresholds sampled from threshold set $\mathbf{\psi} \sim \mathbf{\Psi}$ yields an unbiased estimate of retrieval performance as presented in Equation \ref{eq:eval}.
\end{theorem}



